Generating Hierarchical Explanations on Text Classification via Feature Interaction Detection

Generating explanations for neural networks has become crucial for their applications in real-world with respect to reliability and trustworthiness. In natural language processing, existing methods usually provide important features which are words or phrases selected from an input text as an explanation, but ignore the interactions between them. It poses challenges for humans to interpret an explanation and connect it to model prediction. In this work, we build hierarchical explanations by detecting feature interactions. Such explanations visualize how words and phrases are combined at different levels of the hierarchy, which can help users understand the decision-making of black-box models. The proposed method is evaluated with three neural text classifiers (LSTM, CNN, and BERT) on two benchmark datasets, via both automatic and human evaluations. Experiments show the effectiveness of the proposed method in providing explanations that are both faithful to models and interpretable to humans.

==> Makefile <==
### latex.makefile
# Author: Jason Hiebel

PROJECT = main

# This is a simple makefile for compiling LaTeX documents. The core assumption
# is that the resulting documents should have any parameters effecting
# rendering quality set to theoretical limits and that all fonts should be
# embedded. While typically overkill, the detriment to doing so is negligible.

# Targets:
#    default : compiles the document to a PDF file using the defined
#              latex generating engine. (pdflatex, xelatex, etc)
#    display : displays the compiled document in a common PDF viewer.
#              (currently linux = evince, OSX = open)
#    clean   : removes the obj/ directory holding temporary files

default: obj/$(PROJECT).pdf

display: default
	(${PDFVIEWER} obj/$(PROJECT).pdf &)


### Compilation Flags
PDFLATEX_FLAGS  = -halt-on-error -output-directory obj/

TEXINPUTS = .:obj/
TEXMFOUTPUT = obj/


### File Types (for dependancies)
TEX_FILES = $(shell find . -name '*.tex' -or -name '*.sty' -or -name '*.cls')
BIB_FILES = $(shell find . -name '*.bib')
BST_FILES = $(shell find . -name '*.bst')
IMG_FILES = $(shell find . -path '*.jpg' -or -path '*.png' -or \( \! -path './obj/*.pdf' -path '*.pdf' \) )


### Standard PDF Viewers
# Defines a set of standard PDF viewer tools to use when displaying the result
# with the display target. Currently chosen are defaults which should work on
# most linux systems with GNOME installed and on all OSX systems.

UNAME := $(shell uname)

ifeq ($(UNAME), Linux)
PDFVIEWER = evince
endif

ifeq ($(UNAME), Darwin)
PDFVIEWER = open
endif


### Clean
# This target cleans the temporary files generated by the tex programs in
# use. All temporary files generated by this makefile will be placed in obj/
# so cleanup is easy.

clean::
	rm -rf obj/

### Core Latex Generation
# Performs the typical build process for latex generations so that all
# references are resolved correctly. If adding components to this run-time
# always take caution and implement the worst case set of commands.
# Example: latex, bibtex, latex, latex
#
# Note the use of order-only prerequisites (prerequisites following the |).
# Order-only prerequisites do not effect the target -- if the order-only
# prerequisite has changed and none of the normal prerequisites have changed
# then this target IS NOT run.
#
# In order to function for projects which use a subset of the provided features
# it is important to verify that optional dependancies exist before calling a
# target; for instance, see how bibliography files (.bbl) are handled as a
# dependency.

obj/:
	mkdir -p obj/

obj/$(PROJECT).aux: $(TEX_FILES) $(IMG_FILES) | obj/
	pdflatex $(PDFLATEX_FLAGS) $(PROJECT)

obj/$(PROJECT).bbl: $(BIB_FILES) | obj/$(PROJECT).aux
	bibtex obj/$(PROJECT)
	pdflatex $(PDFLATEX_FLAGS) $(PROJECT)

obj/$(PROJECT).pdf: obj/$(PROJECT).aux $(if $(BIB_FILES), obj/$(PROJECT).bbl)
	pdflatex $(PDFLATEX_FLAGS) $(PROJECT)


==> alg-inter-shap.tex <==
\begin{algorithm}[htbp]
  \begin{algorithmic}[1]
    \State{\textbf{Input:} an input text $\mathbf{x}$ with length $n$}
    \State{Initialize hierarchy $\mathbf{h}$, $\mathcal{N}=\{1,\ldots,n\}$}
    \State{set $p=0$, $\mathbf{x}=[\mathbf{x}]$}
    \While{$p<len(\mathbf{x})$}
    \State{$\mathbf{z}=\mathbf{x}[p]$, $\mathbf{r}=\mathbf{x}$}
    \If{$len(\mathbf{z})==1$}
    \State{$p=p+1$}
    \State{\textbf{continue}}
    \EndIf
    \For{$i=0:len(\mathbf{z})-2$}
    \State{$\mathbf{z}_l=\mathbf{z}[0:i]$, $\mathbf{z}_r=\mathbf{z}[i+1:len(\mathbf{z})-1]$}
    \State{delete $\mathbf{z}$ from $\mathbf{r}$}
    \State{Insert $\mathbf{z}_l$ into $\mathbf{r}$ at $p$-th position}
    \State{Insert $\mathbf{z}_r$ into $\mathbf{r}$ and $p+1$-th position}
    \State{Compute $\psi^i_{p(p+1)}(\mathbf{r})$}
    \EndFor
    \State{$p^*=\arg\min_i\psi^i_{p(p+1)}(\mathbf{r}), i=0,\ldots,len(\mathbf{z})-2$}
    \State{$\gamma=\min_i\psi^i_{p(p+1)}(\mathbf{r}), i=0,\ldots,len(\mathbf{z})-2$}
    \State{Delete $\mathbf{z}$ from $\mathbf{x}$}
    \State{$\mathbf{z}_l=\mathbf{z}[0:p^*]$, $\mathbf{z}_r=\mathbf{z}[p^*+1:len(\mathbf{z})-1]$}
    \State{Insert $\mathbf{z}_l$ into $\mathbf{x}$ at $p^*$-th position}
    \State{Insert $\mathbf{z}_r$ into $\mathbf{x}$ and $p^*+1$-th position}
    \State{$\mathbf{h}$.add($\mathbf{z}_l$, $\mathbf{z}_r$)}
    \EndWhile
    \State{\Return{$\mathbf{h}$}}
  \end{algorithmic}
  \caption{Top-down segmentation algorithm.}
  \label{alg:inter-shap}
\end{algorithm}

==> background.tex <==
\section{Background and Preliminaries}
\label{sec:background}

In this section, we introduce some background on Shapley-based values, and their applications in additive feature attribution methods.

\subsection{Shapley value}
\label{sec:shapley_value}
Shapley value~\citep{shapley1953value} is a concept from coalitional game theory, where the worth of a grand coalition is distributed to each player in a "fair" way. Shapley value provides a solution to calculate the payoff of a player ($i$) as,

\begin{small}
\begin{align}
\label{eq:shapleyvalue}
\phi(i)=\sum_{S\subseteq \mathcal{N}\backslash\{i\}}\frac{|S|!(n-|S|-1)!}{n!}(v(S\cup\{i\})-v(S)),
\end{align}
\end{small}
where $\mathcal{N}=\{1, 2, ..., n\}$ is a finite set of $n$ players, $|S|$ is the number of players in the subset $S$, and $v(\cdot)$ is a characteristic function, with $v(\emptyset)=0$ and $\sum_{i\in \mathcal{N}}\phi(i)=v(\mathcal{N})$ (\textbf{efficiency axiom})~\citep{vstrumbelj2014explaining, kononenko2010efficient}. The difference between $v(S\cup\{i\})$ and $v(S)$ is usually called the marginal contribution of $i$ to $S$.

\subsection{Shapley interaction index}
\label{sec:shapley_interaction}
\citet{grabisch1999axiomatic} noticed that in general, $\phi(i)$ is not equal to $v(i)$, which means that the player $i$ has some joint interest with other players in forming coalitions. For example, cosidering another player $j$, if $v(i, j)>v(i) + v(j)$, then there is a positive interaction between $i$ and $j$. The Shapley interaction index~\citep{owen1972multilinear, grabisch1997k, fujimoto2006axiomatic} is defined to measure the interaction between $i$ and $j$ as,

\begin{small}
	\begin{align}
	\label{eq:shapleyinteraction}
	\phi(i, j)=\sum_{S\subseteq \mathcal{N}\backslash\{i, j\}}\frac{|S|!(n-|S|-2)!}{(n-1)!}\gamma_{i, j}(v),
	\end{align}
\end{small}
where $\gamma_{i, j}(v)=v(S\cup \{i, j\})- v(S\cup \{i\})- v(S\cup\{j\})+v(S)$ can be regarded as the difference between the marginal contributions.

\citet{lundberg2018consistent} first applied Shapley interaction index to SHAP interaction values to calculate feature attributions for tree ensembles. We extend this method to build model-agnostic hierarchical explanations for any black-box models in \autoref{sec:method}.

\subsection{Additive feature attribution methods}
\label{sec:additivemethod}
For a complex neural network model $f$, \citet{ribeiro2016should} proposed a local interpretation method, LIME, to explain the prediction $f(x)$ of each single input $x$. \citet{lundberg2017unified} concluded it with other similar methods (e.g., DeepLIFT~\citep{shrikumar2017learning}) into a unified additive feature attribution method,
\begin{align}
\label{eq:unifiedequ}
g(z')=\phi_{0}+\sum_{i=1}^{n}\phi_{x}(i)z_{i}',
\end{align}
where $z'\in\{0, 1\}^{n}$ is a subsample of the binary representation ($x'$) of the input $x$, with $0$ and $1$ representing the absence or presence of a feature. The goal is to make $g(z')\approx f(h_{x}(z'))$, where $h_{x}(\cdotp)$ maps the binary representation to the original input. The obtained weights $\{\phi_{x}(1), \phi_{x}(2), \cdots, \phi_{x}(n)\}$ are the contributions of input variables $\{x_{1}, x_{2}, \cdots, x_{n}\}$ to the model prediction. Shapley value has been demonstrated as the optimal solution to compute feature attributions, with $v(\cdotp)=f(\cdotp)$ in \autoref{eq:shapleyvalue} and each feature $x_{i}$ is a player in the coalition game \citep{lundberg2017unified}.

Although Shapley value $\phi_{x}(i)$ exactly computes the feature attribution by exhaustively counting the contributions of $i$ in all $2^{(n-1)}$ subsets that contain it, the exponential computational complexity makes this problem intractable. Various approximation methods have been proposed to reduce complexity: SampleShapley~\citep{kononenko2010efficient} by applying sampling approximations, KernelSHAP~\citep{lundberg2017unified} by using a weighted linear regression, and L/C-Shapley~\citep{chen2018shapley} by only considering the local or connected neighbour features. We address this problem by calculating Shapley-based values on N-gram features in \autoref{sec:method}.

==> tab-datasets.tex <==
\begin{table}
  \centering
  \begin{tabular}{p{0.15\textwidth}lllll}
    	\toprule
         Dataset & Classes & Average length & Train & Dev. & Test \\
         \midrule
         SST-2 & 2 & 19 & 6920 & 872 & 1821 \\
         % \hline
         IMDB & 2 & 268 & 22500 & 2500 & 25000 \\
         \bottomrule
  \end{tabular}
  \caption{Summary statistics for the datasets.}
  \label{tab:datasets}
\end{table}

==> tab-models.tex <==
 \begin{table*}
   \centering
   \begin{tabular}{lll}
     \toprule
     Datasets & Models & Accuracy \\
     \midrule
     \multirow{3}{*}{SST} &  &  \\
                          & LSTM & 0.842 \\
                          & CNN & 0.850  \\
                          & BERT & 0.924  \\
 	\emph{}
 	\multirow{3}{*}{IMDB} &  &   \\
 						 & LSTM & 0.870  \\
 						 & CNN & 0.901 \\
 						 & BERT & 0.930  \\
     \bottomrule
   \end{tabular}
   \caption{The classification results of different models on SST and IMDB.}
   \label{tab:models}
\end{table*}

==> tables/tab-datasets.tex <==
\begin{table}[tbph]
  \centering
  \begin{tabular}{p{0.12\textwidth}lll}
    	\toprule
         Dataset & \textit{C} & \textit{L} & \textit{N} \\
         \midrule
         SST & 2 & 19 & 9613 \\
         % \hline
         IMDB & 2 & 268 & 50000 \\
         \bottomrule
  \end{tabular}
  \caption{Summary statistics for the datasets, where \textit{C} is the number of classes, \textit{L} is average sentence length, and \textit{N} is dataset size.}
  \label{tab:datasets}
\end{table}
